Tightened Convex Relaxations for Neural Network Robustness Certification

In this paper, we consider the problem of certifying the robustness of neural networks to perturbed and adversarial input data. Such certification is imperative for the application of neural networks in safety-critical decision-making and control systems. Certification techniques using convex optimization have been proposed, but they often suffer from relaxation errors that void the certificate. Our work exploits the structure of ReLU networks to improve relaxation errors through a novel partition-based certification procedure. The proposed method is proven to tighten existing linear programming relaxations, and asymptotically achieves zero relaxation error as the partition is made finer. We develop a finite partition that attains zero relaxation error and use the result to derive a tractable partitioning scheme that minimizes the worst-case relaxation error. Experiments using real data show that the partitioning procedure is able to issue robustness certificates in cases where prior methods fail. Consequently, partition-based certification procedures are found to provide an intuitive, effective, and theoretically justified method for tightening existing convex relaxation techniques.

==> sections/notes.tex <==
\subsection{Strictly decreasing objectives}
Note that in Proposition \ref{prop: decreasing_objective}, we only show that upon partitioning the relaxation, the relaxation bound is at least as tight as the original unpartitioned relaxation. It is our hope to extend this result to give sufficient conditions for when partitioning leads to a \emph{strictly decreasing} objective. As a first approach to this extension, we provide some intuition on the partitioned LP relaxations:

The inequality (\ref{eq: decreasing_objective}) will hold strictly when $f^*(\mathcal{X})<\hat{f}^*(\mathcal{X})$ (otherwise the original relaxation is already exact) and the partition sufficiently reduces some of the error associated with the relaxation. We note that when $f^*(\mathcal{X})<\hat{f}^*(\mathcal{X})$ and $(x^*,z^*)$ denotes an optimal solution for $\hat{f}^*(\mathcal{X})$, it must be the case that there exists some coordinate $k\in\{1,2,\dots,n_z\}$ such that
\begin{equation*}
z^*_k = \frac{u_k}{u_k-l_k}(w_k^\top x^* - l_k),
\end{equation*}
for otherwise $z^*=\relu(Wx^*)$ (which contradicts the inexact relaxation) or one can set $z^*_k$ equal to the above expression and strictly increase the objective (which contradicts the optimality of $z^*$). Therefore, it is our conjecture that choosing a partition $\{\mathcal{X}_i : i\in\{1,2,\dots,p\}\}$ such that $l_k<l_k^{(i)}$, $u_k^{(i)}<u_k$, $l\le l^{(i)}$, and $u^{(i)}\le u$ for all $i\in\{1,2,\dots,p\}$, we should find that the $k$th coordinate of the $i$th partition should ``move down'' with the upper bound $g^{(i)}_k(x) = \frac{u_k^{(i)}}{u_k^{(i)}-l_k^{(i)}}(w_k^\top x - l_k^{(i)})$ since $g^{(i)}_k(x)<g_k(x) = \frac{u_k}{u_k-l_k}(w_k^\top x - l_k)$. We predict that such a strict decrease in the $k$th coordinate of $z$ at optimality should yield the strict decrease in the optimal objective value we desire. We have yet to formally prove this conjecture.

\subsection{Optimal partitioning}
In Theorem \ref{thm: worst-case_relaxation_bound} and Corollary \ref{cor: optimal_worst-case_partition}, we use a worst-case scenario analysis to characterize the best partitioning scheme (of those based on the rows of $W$). In general, the errors introduced by the relaxation will not all be as large as possible, and therefore the worst-case analysis used is overly conservative. We'd like to be able to find an optimal partition based on the rows of $W$ that holds in the true sense. That is, performing such partition should be guaranteed to tighten the relaxation as much as possible among all other possible partitions based on the rows of $W$.

As a first approach to solving this problem, suppose a coordinate $k$ satisfies $z^*_k=0$ or $z^*_k = w_k^\top x^*$, where $(x^*,z^*)$ is an optimal point of the unpartitioned relaxation. Then clearly, performing the partition based on $w_k$ (i.e.\ $w_k^\top x\ge 0$ in the first part and $w_k^\top x < 0$ in the second part) is a poor choice, since the optimal point already satisfies $z_k^*=\relu(w_k^\top x^*)$. Hence, partitioning via the $k$th row of $W$ redundantly ensures the relaxation is exact in the $k$th coordinate.

Instead, we should only consider partitioning according to row $k$ of $W$ if $z_k^* > 0$ and $z^*_k > w_k^\top x^*$ in the unpartitioned relaxation. For such $k$, it must hold that $z^*_k = \frac{u_k}{u_k-l_k}(w_k^\top x^* - l_k)$ for the unpartitioned solution. Using this property of all of the inexact coordinates, we seek to determine which coordinate would result in the largest decrease in the objective value upon partitioning based on its corresponding row in $W$. We conjecture that the optimal row should be of some form similar to
\begin{equation*}
k^* \in \arg\max_{k\in\{1,2,\dots,n_z\}} c_k(z^*_k - \relu(w_k^\top x^*)),
\end{equation*}
where $z^*$ solves the unpartitioned relaxation. Such type of result remains to be formally proven.

==> sections/partitioned_relaxation_error.tex <==
In this section, we discuss the effect of partitioning on the relaxation error. If we linearly decrease the bound on the input $x$ by a factor $t \in \{\mathbb{R}|t \in (0,1)\}$, we hope to know how the relaxation gap (difference between relaxed objective and un-relaxed objective) change. Especially we want to have a function of the difference in gap in terms of $t$. Since in the best-case scenario the un-partitioned relaxation will be tight, we'll discuss this problem in a worst-case scenario sense.

For each coordinate k of $z_k$, the value can only increase or decrease. Whether it increases or decreases depend on the gradient direction of the cost function $c^\top x$. Since this is a maximization problem, $z$ will go in the positive gradient direction, thus $c$. Therefore if $c_k$ is positive, $z_k$ will try to increase as much as possible, and the other direction also holds.

Therefore,
\begin{equation*}
\begin{aligned}{}
\sup_{z_k} &= u_k \ \forall \ \ k \in K^+ = \{1,\dots,n_z |  c_k > 0\}  \\
\inf_{z_k} &= 0  \ \forall \ \ k \in K^- =  \{1,\dots,n_z |  c_k < 0\}
\end{aligned}
\end{equation*}{}
When suprema are achieved for coordinates in $K^+$ and infima are achieved for coordinates in $K^-$, the maximum possible value of $ f^*(\mathcal{X})$ is achieved given $l$ and $u$, and we denote it as $f^*(\mathcal{X})_{\max}$. This corresponds to the "worst-case scenario" because this is the loosest upper bound we can have. 

Now we consider the effect of the scaling of $\mathcal{X}$ on $f^*(\mathcal{X})_{\max}$. In particular, if we scale the bounds on $\mathcal{X}$ by the factor $t$, and denote this new input space as $\mathcal{X}_t$, how would $f^*(\mathcal{X}_t)_{\max}$ compare to $f^*(\mathcal{X})_{\max}$?

With $\mathcal{X}_t$,
\begin{equation*}
\begin{aligned}{}
\sup_{z_k} &= t*u_k \ \forall \ \ k \in K^+ = \{1,\dots,n_z |  c_k > 0\}  \\
\inf_{z_k} &= 0  \ \forall \ \ k \in K^- =  \{1,\dots,n_z |  c_k < 0\}
\end{aligned}
\end{equation*}{}

Thus,
\begin{equation*}
f^*(\mathcal{X})_{\max} - f^*(\mathcal{X}_t)_{\max} \geq (1-t)c_{K^+}^\top u_{K^+}
\end{equation*}{}
where $c_{K^+} = [c_j | j \in K^+]$, and $u_{K^+} = [u_j | j \in K^+]$.

This gives a lower-bound on the reduction in relaxation error in the "worst-case scenario" as explained above.

{\color{red}
	
	Given $(x,z)\in\mathcal{N}$, the output $z_i$ is upper bounded by the line $g_i(x) = \frac{u_i}{u_i-l_i} (w_i^\top x - l_i)$ and lower bounded by $\relu(w_i^\top x)$. Therefore, for a fixed $x\in\mathcal{X}$ we have that
	\begin{multline*}
	\sup_{z\in\{z : (x,z)\in\mathcal{N}\}} (z_i - \relu(w_i^\top x)) = \\
	\begin{aligned}
	\begin{cases}
	\left(\frac{u_i}{u_i-l_i}-1\right)w_i^\top x - \frac{u_i l_i}{u_i-l_i} & \text{if $w_i^\top x \ge 0$}, \\
	\frac{u_i}{u_i-l_i}w_i^\top x - \frac{u_i l_i}{u_i-l_i} & \text{if $w_i^\top x < 0$}.
	\end{cases}
	\end{aligned}
	\end{multline*}
	
	Now consider the partitioning effect. In the simplest case, we shrink the bound of the input by a scaling factor, i.e. $l'_i = t l_i, u'_i = t u_i, t \in (0,1)$. Note that these are bounds for the pre-activation $\hat z_i$. Since we are originally partitioning $x$, and $\hat z$ is just a linear transformation of $x$, the scaling factor of the bounds on $x$ carries over. Of course the more general case would be that each bound has a different scaling factor, but as you'd see below that won't really effect the analysis much and the use of the same factor would simplify notation significantly.
	
	In this case, we would calculate the maximum error after partition as
	\begin{align*}
	\max_{\text{partitioned}}\{z_i-x_i\} &=  (\frac{u_i}{u_i-l_i} -1) w_i x_i - t \frac{u_i l_i}{u_i -l_i} \\
	\text{or} &= \frac{u_i}{u_i-l_i}  w_i x_i - t \frac{u_i l_i}{u_i -l_i}
	\end{align*}{}
	In both cases,
	\begin{align*}
	&\max\{z_i-x_i\} - \max_{\text{partitioned}}\{z_i-x_i\} \\
	=& \max z_i - \max_{\text{partitioned}} z_i\\
	=& (t-1) \frac{u_i l_i}{u_i -l_i}
	\end{align*}
	Note $u_i l_i$ is negative, so smaller the $t$ is, bigger the gap.
	
	From this derivation we can find that the reduction in error in LP goes up linearly with t. However, the absolute value in reduction depends on the magnitude of the bounds. With bounds bigger in absolute value, we get more reduction in relaxation error. Therefore this tells us that input partitioning works best with loose bounds.
	
	Furthermore, we can extend this notion in a multi-layer setting. Imagine $x_i^{L=2} = z_i^{L=1}$ is the ith input in the second layer. With partitioning at the input layer, $x_{i_{\text{partitioned}}}^{L=2} = x_i^{L=2} - (t-1) \frac{u_i l_i}{u_i -l_i}$. Thus subsequently (for $w_i x > 0$),
	\begin{align*}
	&\max_{\text{partitioned}}\{z_{i}^{L=2}-x_{i}^{L=2}\} \\
	&= (\frac{u_i}{u_i-l_i} -1) w_i x_{i_{\text{partitioned}}}^{L=2} \\
	&- t \frac{u_i l_i}{u_i -l_i} \\
	&= (\frac{u_i}{u_i-l_i} -1) w_i (x_i^{L=2} + (1-t) \frac{u_i l_i}{u_i -l_i}) \\
	&- t \frac{u_i l_i}{u_i -l_i} \\
	&= (\frac{u_i}{u_i-l_i} -1) w_i x_i^{L=2} - t \frac{u_i l_i}{u_i -l_i} \\
	&+ (\frac{u_i}{u_i-l_i} -1) (1-t) \frac{u_i l_i}{u_i -l_i}
	\end{align*}{}
	This assumes that we use the same upper and lower bounds for the second layer. In reality, these bounds may shrink with simple arithmetic tricks. However, to analyze this issue in the worst-case scenario, and to make the derivations as clean as possible, we'll use the same bounds for all layers. Increasingly tight bounds (the usual practice) would yield tighter relaxations. Therefore, similarly,
	\begin{align*}
	&\max\{z_i^{L=2}-x_i^{L=2}\} - \max_{\text{partitioned}}\{z_i^{L=2}-x_i^{L=2}\} \\
	=& \max z_i^{L=2} - \max_{\text{partitioned}} z_i^{L=2}\\
	=& (t-1)  \frac{u_i l_i}{u_i -l_i}(1+(\frac{u_i}{u_i-l_i} -1))
	\end{align*}{}
	By induction,
	\begin{align*}
	&\max z_i^{L=n} - \max_{\text{partitioned}} z_i^{L=n}\\
	&= (t-1)  \frac{u_i l_i}{u_i -l_i} \\
	&(1+(\frac{u_i}{u_i-l_i} -1)+...+(\frac{u_i}{u_i-l_i} -1)^{n-1})
	\end{align*}{}
	If we define $(\frac{u_i}{u_i-l_i} -1) = \gamma$, then
	\begin{align*}
	\max z_i^{L=n} - \max_{\text{partitioned}} z_i^{L=n} &= (t-1)\frac{1-\gamma^n}{1-\gamma} \frac{u_i l_i}{u_i -l_i} \\
	&= (t-1)(1-\gamma^n)\frac{u_i l_i}{u_i-2l_i}
	\end{align*}{}
	When $l_i \leq 0$, $|\gamma^n| \leq 1$. Therefore error reduction is still linearly dependent on t, but its absolute magnitude is heavily dependent on $\frac{u_i l_i}{u_i-2l_i}$. Again, as with single layers analysis, input partitioning works best with looser bounds. However, what this tells us is that the number of layers in the network is not a huge factor in the amount of relaxation error reduction when input partitioning is applied.
	
	
}

==> sections/preactivation_bounds.tex <==
In this section, we present various computational approaches for approximating preactivation bounds. We show a simple method for approximating the preactivation bounds at layer $k+1$ given those at layer $k$. Furthermore, we present two methods for computing the first layer's preactivation bounds in the case the input uncertainty set is a $\ell_\infty$-ball.

\begin{proposition}[Preactivation bound computation]
\label{prop: preactivation_bound_computation}
Let $l^{[k]},u^{[k]}\in\mathbb{R}^{n_k}$ be valid preactivation bounds for layer $k\in\{1,2,\dots,K\}$. Then
\begin{equation}
    \begin{aligned}
    l^{[k+1]} ={}& \min\left\{0,\max\{0,W^{[k]}\}l^{[k]} + \min\{0,W^{[k]}\}u^{[k]}\right\}, \\
    u^{[k+1]} ={}& \max\left\{0,\max\{0,W^{[k]}\}u^{[k]} + \min\{0,W^{[k]}\}l^{[k]}\right\},
    \end{aligned} \label{eq: preactivation_bound_computation}
\end{equation}
are valid preactivation bounds for layer $k+1$.
\end{proposition}

\begin{proof}
We have that
\begin{equation}
    \begin{aligned}
    \hat{z}^{[k+1]} ={}& W^{[k]}x^{[k]} \\
    ={}& W^{[k]}\max\{0,\hat{z}^{[k]}\} \\
    ={}& \max\{0,W^{[k]}\}\max\{0,\hat{z}^{[k]}\} \\
    &{}+ \min\{0,W^{[k]}\}\max\{0,\hat{z}^{[k]}\}.
    \end{aligned} \label{eq: preactivation_bound_computation_intermediate_0}
\end{equation}
Now, noting that $l^{[k]}\le \hat{z}^{[k]}\le u^{[k]}$ and $l^{[k]}\le 0 \le u^{[k]}$, we find the following inequalities:
\begin{enumerate}
    \item Since $\max\{0,\hat{z}^{[k]}\} \ge l^{[k]}$ and $\max\{0,W^{[k]}\}\ge 0$,
    \begin{equation}
        \max\{0,W^{[k]}\}\max\{0,\hat{z}^{[k]}\} \ge \max\{0,W^{[k]}\}l^{[k]}. \label{eq: preactivation_bound_computation_intermediate_1}
    \end{equation}
    \item Since $\max\{0,\hat{z}^{[k]}\} \le u^{[k]}$ and $\min\{0,W^{[k]}\}\le 0$,
    \begin{equation}
        \min\{0,W^{[k]}\}\max\{0,\hat{z}^{[k]}\} \ge \min\{0,W^{[k]}\}u^{[k]}. \label{eq: preactivation_bound_computation_intermediate_2}
    \end{equation}
    \item Since $\max\{0,\hat{z}^{[k]}\} \le u^{[k]}$ and $\max\{0,W^{[k]}\}\ge 0$,
    \begin{equation}
        \max\{0,W^{[k]}\}\max\{0,\hat{z}^{[k]}\} \le \max\{0,W^{[k]}\}u^{[k]}. \label{eq: preactivation_bound_computation_intermediate_3}
    \end{equation}
    \item Since $\max\{0,\hat{z}^{[k]}\} \ge l^{[k]}$ and $\min\{0,W^{[k]}\}\le 0$,
    \begin{equation}
        \min\{0,W^{[k]}\}\max\{0,\hat{z}^{[k]}\} \le \min\{0,W^{[k]}\}l^{[k]}. \label{eq: preactivation_bound_computation_intermediate_4}
    \end{equation}
\end{enumerate}
Substituting (\ref{eq: preactivation_bound_computation_intermediate_1}) and (\ref{eq: preactivation_bound_computation_intermediate_2}) into (\ref{eq: preactivation_bound_computation_intermediate_0}) yields
\begin{equation*}
    \hat{z}^{[k+1]} \ge \max\{0,W^{[k]}\}l^{[k]} + \min\{0,W^{[k]}\}u^{[k]},
\end{equation*}
and substituting (\ref{eq: preactivation_bound_computation_intermediate_3}) and (\ref{eq: preactivation_bound_computation_intermediate_4}) into (\ref{eq: preactivation_bound_computation_intermediate_0}) yields
\begin{equation*}
    \hat{z}^{[k+1]} \le \max\{0,W^{[k]}\}u^{[k]} + \min\{0,W^{[k]}\}l^{[k]},
\end{equation*}
proving the validity of the preactivation bounds proposed in (\ref{eq: preactivation_bound_computation}).
\end{proof}

\begin{proposition}[Preactivation bounds for $\ell_\infty$-ball]
\label{prop: preactivation_bounds_l_infty}
Suppose the input uncertainty set is $\mathcal{X} = \{x\in\mathbb{R}^{n_x} : \|x-\bar{x}\|_{\infty} \le \epsilon\}$. Then the preactivation bounds can be taken as
\begin{equation}
    \begin{aligned}
    l^{[1]} ={}& \min\Big\{0,W^{[0]}\bar{x} - \epsilon \max\{0,W^{[0]}\}\mathbf{1}_{n_x} \\
    &{}+ \epsilon \min\{0,W^{[0]}\}\mathbf{1}_{n_x}\Big\}, \\
    u^{[1]} ={}& \max\Big\{0,W^{[0]}\bar{x} + \epsilon \max\{0,W^{[0]}\}\mathbf{1}_{n_x} \\
    &{}- \epsilon \min\{0,W^{[0]}\}\mathbf{1}_{n_x}\Big\},
    \end{aligned} \label{eq: preactivation_bounds_l_infty}
\end{equation}
where $\mathbf{1}_{n_x}$ is the $n_x$-vector of all ones. The remaining bounds $l^{[k]},u^{[k]}$ for $k>1$ can be computed according to (\ref{eq: preactivation_bound_computation}).
\end{proposition}

\begin{proof}
All we must show is the computation for the first layer, i.e.\ $l^{[1]}$ and $u^{[1]}$. We have that
\begin{equation}
    \begin{aligned}
        \hat{z}^{[1]} ={}& W^{[0]x} \\
        ={}& W^{[0]}(x-\bar{x}) + W^{[0]}\bar{x} \\
        ={}& W^{[0]}\bar{x} + \max\{0,W^{[0]}\}\max\{0,x-\bar{x}\} \\
        &{} + \max\{0,W^{[0]}\}\min\{0,x-\bar{x}\} \\
        &{} + \min\{0,W^{[0]}\}\max\{0,x-\bar{x}\} \\
        &{} + \min\{0,W^{[0]}\}\min\{0,x-\bar{x}\}. \label{eq: preactivation_bounds_l_infty_intermediate_0}
    \end{aligned}
\end{equation}
Noting that $-\epsilon\mathbf{1}_{n_x} \le x-\bar{x} \le \epsilon\mathbf{1}_{n_x}$ and $-\epsilon \mathbf{1}_{n_x} \le 0 \le \epsilon \mathbf{1}_{n_x}$, we find the following inequalities:
\begin{enumerate}
    \item Since $\max\{0,x-\bar{x}\}\ge 0$ and $\max\{0,W^{[0]}\} \ge 0$,
    \begin{equation}
        \max\{0,W^{[0]}\}\max\{0,x-\bar{x}\} \ge 0. \label{eq: preactivation_bounds_l_infty_intermediate_1}
    \end{equation}
    \item Since $\min\{0,x-\bar{x}\}\ge -\epsilon\mathbf{1}_{n_x}$ and $\max\{0,W^{[0]}\} \ge 0$,
    \begin{equation}
        \max\{0,W^{[0]}\}\min\{0,x-\bar{x}\} \ge -\epsilon\max\{0,W^{[0]}\}\mathbf{1}_{n_x}. \label{eq: preactivation_bounds_l_infty_intermediate_2}
    \end{equation}
    \item Since $\min\{0,x-\bar{x}\}\le \epsilon\mathbf{1}_{n_x}$ and $\max\{0,W^{[0]}\} \le 0$,
    \begin{equation}
        \min\{0,W^{[0]}\}\max\{0,x-\bar{x}\} \ge \epsilon\min\{0,W^{[0]}\}\mathbf{1}_{n_x}. \label{eq: preactivation_bounds_l_infty_intermediate_3}
    \end{equation}
    \item Since $\min\{0,x-\bar{x}\}\le 0$ and $\min\{0,W^{[0]}\} \le 0$,
    \begin{equation}
        \min\{0,W^{[0]}\}\min\{0,x-\bar{x}\} \ge 0. \label{eq: preactivation_bounds_l_infty_intermediate_4}
    \end{equation}
\end{enumerate}
Substituting (\ref{eq: preactivation_bounds_l_infty_intermediate_1}) through (\ref{eq: preactivation_bounds_l_infty_intermediate_4}) into (\ref{eq: preactivation_bounds_l_infty_intermediate_0}) yields
\begin{equation*}
    \hat{z}^{[1]} \ge W^{[0]}\bar{x} -\epsilon \max\{0,W^{[0]}\}\mathbf{1}_{n_x} + \epsilon\min\{0,W^{[0]}\}\mathbf{1}_{n_x},
\end{equation*}
proving the validity of the preactivation lower bound $l^{[1]}$ proposed in (\ref{eq: preactivation_bounds_l_infty}). Proving the validity of $u^{[1]}$ proposed in (\ref{eq: preactivation_bounds_l_infty}) follows from analogous reasoning.
\end{proof}

\begin{proposition}[Simple preactivation bounds for $\ell_\infty$-ball]
\label{prop: preactivation_bounds_l_infty_simple}
Suppose the input uncertainty set is $\mathcal{X} = \{x\in\mathbb{R}^{n_x} : \|x-\bar{x}\|_\infty \le \epsilon\}$. Then the preactivation bounds can be taken as
\begin{equation}
    \begin{aligned}
    u^{[1]} ={}& |W^{[0]}||\bar{x}| + \epsilon |W^{[0]}|\mathbf{1}_{n_x}, \\
    l^{[1]} ={}& -u^{[1]},
    \end{aligned} \label{eq: preactivation_bounds_l_infty_simple}
\end{equation}
where $\mathbf{1}_{n_x}$ is the $n_x$-vector of all ones. The remaining bounds $l^{[k]},u^{[k]}$ for $k>1$ can be computed according to (\ref{eq: preactivation_bound_computation}).
\end{proposition}

\begin{proof}
All we must show is the computation for the first layer, i.e.\ $l^{[1]}$ and $u^{[1]}$. We have that
\begin{equation*}
    \begin{aligned}
    \hat{z}^{[1]} ={}& W^{[0]}x \\
    \le{}& |W^{[0]}(x-\bar{x}+\bar{x})| \\
    \le{}& |W^{[0]}||\bar{x}| + |W^{[0]}||x-\bar{x}|.
    \end{aligned}
\end{equation*}
Since $|x-\bar{x}|\le \epsilon\mathbf{1}_{n_x}$,
\begin{equation*}
    \hat{z}^{[1]} \le |W^{[0]}||\bar{x}| + \epsilon|W^{[0]}|\mathbf{1}_{n_x},
\end{equation*}
proving the validity of the preactivation upper bound $u^{[1]}$ proposed in (\ref{eq: preactivation_bounds_l_infty_simple}). Proving the validity of the preactivation lower bound $l^{[1]}$ proposed in (\ref{eq: preactivation_bounds_l_infty_simple}) follows from analogous reasoning.
\end{proof}

\begin{remark}
From our simulations, we find the more sophisticated bounds in Proposition \ref{prop: preactivation_bounds_l_infty} to yield tighter relaxations when compared to the simpler bounds in Proposition \ref{prop: preactivation_bounds_l_infty_simple}. However, we use the bounds in Proposition \ref{prop: preactivation_bounds_l_infty_simple} not only due to their simplicity and more intuitive form, but also because the resulting simulations better graphically explain the impact of our results on optimal partitioning.
\end{remark}

==> sections/sdp_results.tex <==
\section{Problem Statement}

Another alternative is to solve a semidefinite program (SDP) relaxation of the problem. In this formulation, the relaxed network constraint set is defined by
\begin{equation}
\begin{aligned}
\mathcal{N}_\text{SDP} ={}& \{P\in\mathbb{R}^{n_x+n_z+1}\times\mathbb{R}^{n_x+n_z+1} : \\
& P[z]\ge 0, ~ P[z]\ge WP[x], \\
& \diag(P[zz^\top]) = \diag(WP[xz^\top]), \\
& \diag(P[xx^\top]) \le (\hat{l}+\hat{u}) \odot P[x] - \hat{l} \odot \hat{u}, \\
& P[1] = 1, ~ P \succeq 0 \}.
\end{aligned} \label{eq: network_constraint_set_sdp}
\end{equation}
Under this formulation the relaxed robustness certification problem becomes
\begin{equation}
\begin{aligned}
\hat{f}^*_\text{SDP}(\mathcal{X}) ={}& \sup\{c^\top P[z] : P \in\mathcal{N}_\text{SDP}, \\
& P[x] \in\mathcal{X} \}.
\end{aligned} \label{eq: sdp_relaxation}
\end{equation}

\begin{remark}
	The notation $P[\cdot]$ is used to index the matrix $P$:
	\begin{equation*}
	P = \begin{bmatrix}
	P[1] & P[x^\top] & P[z^\top] \\
	P[x] & P[xx^\top] & P[xz^\top] \\
	P[z] & P[zx^\top] & P[zz^\top]
	\end{bmatrix}.
	\end{equation*}
	Furthermore, in the SDP formulation, the bounds $\hat{l}, \hat{u}$ denote bounds on the input as opposed to the preactivation bounds in the LP relaxation.
\end{remark}


\section{Properties of Partitioned Relaxations}

\begin{proposition}[Decreasing SDP objective]
	\label{prop: decreasing_sdp_objective}
	Consider a one-layer feedforward neural network. Let $\{\mathcal{X}_i : i\in\{1,2,\dots,p\}\}$ be a partition of $\mathcal{X}$. For the $i$th input part $\mathcal{X}_i$, denote the corresponding input bounds by $l \le l^{(i)} \le x \le u^{(i)} \le u$, where $x\in\mathcal{X}_i$. Then it holds that
	\begin{equation}
	\max_{i\in\{1,2,\dots,p\}} \hat{f}^*_\text{SDP}(\mathcal{X}_i) \le \hat{f}^*_\text{SDP}(\mathcal{X}). \label{eq: decreasing_sdp_objective}
	\end{equation}
\end{proposition}

\begin{proof}
	Let $i\in\{1,2,\dots,p\}$. From the definition of the partition, it holds that $\mathcal{X}_i\subseteq \mathcal{X}$. What remains to be shown is that $\mathcal{N}_{\text{SDP},i} \subseteq \mathcal{N}_\text{SDP}$.
	
	Let $P\in\mathcal{N}_{\text{SDP},i}$. Define $u' = u^{(i)}$ and $l' = l^{(i)}$. Since $P \in \mathcal{N}_{\text{SDP},i}$, it follows that
	\begin{align*}
	P[z]\ge{}& 0, \\
	P[z]\ge{}& WP[x], \\
	\diag(P[zz^\top]) ={}& \diag(WP[xz^\top]), \\
	\diag(P[xx^\top]) \leq{}& (l'+u') \odot P[x] - l' \odot u', \\
	P[1] ={}& 1, \\
	P \succeq{}& 0.
	\end{align*}
	To show that $P\in\mathcal{N}_\text{SDP}$, we should show that the above expressions imply that $\diag(P[xx^\top])\le (l+u)\odot P[x] - l\odot u$. To do so, define $\Delta l_k\ge 0$ and $\Delta u_k \ge 0$ such that $l_k' = l_k + \Delta l_k$ and $u_k' = u_k - \Delta u_k$ for all $k \in \{1,2,\dots,n_x\}$. To simplify notation, define $x_k = P[x]_k$. Then we find that 
	\begin{align*}
	& ((l'+u') \odot P[x] - l' \odot u')_k \\
	&{}= (l_k'+u_k')x_k-l_k' u_k' \\
	&{}= (l_k+u_k)x_k - l_k u_k + (\Delta l_k - \Delta u_k)x_k \\
	& \quad - ( \Delta l_k u_k - \Delta u_k l_k - \Delta u_k \Delta l_k) \\
	&= ((l+u) \odot P[x] - l \odot u)_k + (\Delta l_k - \Delta u_k)x_k \\
	&\quad - ( \Delta l_k u_k - \Delta u_k l_k - \Delta u_k \Delta l_k).
	\end{align*}
	Therefore, it suffices to prove that $\Delta_k \coloneqq (\Delta l_k - \Delta u_k)x_k - ( \Delta l_k u_k - \Delta u_k l_k - \Delta u_k \Delta l_k) \leq 0$ for all $k$. Since $-l_k u_k \ge -l_k' u_k'$ by definition, it holds that $ \Delta l_k u_k - \Delta u_k l_k - \Delta u_k \Delta l_k \ge 0$. Thus, when $(\Delta l_k - \Delta u_k)x_k \le 0$, it holds that $\Delta_k \leq 0$, as desired. On the other hand, suppose that $(\Delta l_k - \Delta u_k)x_k \ge 0$. Then we find two cases:
	\begin{enumerate}
		\item $(\Delta l_k - \Delta u_k) \ge 0$ and $x_k \ge 0$: The maximum positive value of $(\Delta l_k - \Delta u_k)x_k$ is $(\Delta l_k - \Delta u_k)u'_k$. Therefore, the maximum value of $\Delta_k$ is
		\begin{align*}
		& (\Delta l_k - \Delta u_k)u'_k - ( \Delta l_k u_k - \Delta u_k l_k - \Delta u_k \Delta l_k) \\
		&{}= \Delta l_k(u'_k-u_k)-\Delta u_k u'_k + \Delta u_k l_k + \Delta u_k \Delta l_k \\
		&{}= \Delta l_k (-\Delta u_k) + \Delta u_k \Delta l_k -\Delta u_k u'_k + \Delta u_k l_k \\
		&{}= -\Delta u_k u'_k + \Delta u_k l_k.
		\end{align*}
		Both of the two final terms are nonpositive, and therefore $\Delta_k \le 0$.
		
		\item $(\Delta l_k - \Delta u_k) \le 0$ and $x_k \le 0$: The maximum positive value of $(\Delta l_k - \Delta u_k)x_k$ is $(\Delta l_k - \Delta u_k)l_k'$. Similarly, the maximum value of  $\Delta_k$ is
		\begin{align*}
		& (\Delta l_k - \Delta u_k)l'_k - ( \Delta l_k u_k - \Delta u_k l_k - \Delta u_k \Delta l_k) \\
		&{}= - \Delta u_k \Delta l_k + \Delta u_k \Delta l_k +\Delta l_k l'_k - \Delta l_k u_k \\
		&{}= \Delta l_k l'_k - \Delta l_k u_k.
		\end{align*}
		Both of the two final terms are nonpositive, and therefore $\Delta_k \le 0$.
	\end{enumerate}
	Hence, we find that $(l'+u') \odot P[x] - l' \odot u' \leq (l+u) \odot P[x] - l \odot u$, proving that $P\in\mathcal{N}_\text{SDP}$, and therefore $\mathcal{N}_{\text{SDP},i} \subseteq \mathcal{N}_\text{SDP}$.
	
	Since $\mathcal{X}_i\subseteq \mathcal{X}$ and $\mathcal{N}_{\text{SDP},i} \subseteq \mathcal{N}_\text{SDP}$, it holds that the solution to the problem over the smaller feasible set lower bounds the original solution: $\hat{f}^*_\text{SDP}(\mathcal{X}_i) \le \hat{f}^*_\text{SDP}(\mathcal{X})$. Finally, since $i$ was chosen arbitrarily, this implies the desired inequality (\ref{eq: decreasing_sdp_objective}).
\end{proof}

\section{Partitioned Relaxation Error}
Motivated by \cite{raghunathan2018semidefinite}, we study how $ \hat{f}^*_\text{SDP}(\mathcal{X})$ changes as we decrease $\epsilon$ in the input uncertainty set $\mathcal{X}=\{x\in\mathbb{R}^{n_x}:\|x-\bar{x}\|_\infty\le\epsilon\}$ through a geometric perspective.
	
	First of all, we consider the $P$ matrix as defined in (\ref{eq: network_constraint_set_sdp}). Since it is a symmetric matrix, it allows a factorization as such: $P = VV^\top$. We further define $V$ as such:
	\begin{equation}
	V = \begin{bmatrix}
	\vec{e}^\top \\
	\vec{x_1}^\top \\
	... \\
	\vec{x_{n_x}}^\top \\
	\vec{z_1}^\top \\
	... \\
	\vec{z_{n_z}}^\top
	\end{bmatrix} \in \mathbb{R}^{(1+n_x+n_z) \times 2}, \|\vec{e}\|^2 = 1 
	\end{equation}{}
	Note each vector in V belongs to $\mathbb{R}^2$. If defined this way, then we can interpret entries of $P$ as dot products between vectors, giving us a way to geometrically explain the relationship between $x$ and $z$. For example, $P[1] = \vec{e} \cdot \vec{e}$, $P[x_i] = \vec{x_i} \cdot \vec{e}$, $P[z_i] = \vec{z_i} \cdot \vec{e}$, and  $\diag(P(xx^\top))_i = \vec{x_i} \cdot \vec{x_i}$. Now we break down the constraints on $P$ to see how $\epsilon$ influences $ \hat{f}^*_\text{SDP}(\mathcal{X})$.
	
	\begin{enumerate}
		\item Input constraints \\
		The input constraint ($x \in \mathcal{X}$) $\diag(P[xx^\top]) \leq (l+u)\odot P[x] - l \odot u$ can be interpreted as $\|\vec{x_i}\|^2 \leq (l_i+u_i)(\vec{x_i} \cdot \vec{e})-l_i u_i \ \forall i \in \{1 . . . n_x\}$. For each $x_i$, this translates to a sphere with centre at $\frac{1}{2}(l_i+u_i)\vec{e}$ and radius $\frac{1}{2} (l_i-u_i)$ in the geometrical space.
		\item ReLU constraints \\
		The constraint $\diag(P[zz^\top]) = \diag(WP[xz^\top])$ is equivalent to $\|\vec{z_i}\|^2 = \langle \vec{p_i} ,\vec{z_i} \rangle \ \forall i \in {1,\dots,n_z}$, where $\vec{p_i} = w_{i1} \vec{x_1}+\dots+w_{in_x}\vec{x_{n_x}}$, and $\langle \cdot, \cdot \rangle$ denotes standard vector inner product. Therefore $\vec{p_i}$ is just a weighted sum of the $\vec{x_{1\dots n_x}}$ vectors with weights being the $i^{th}$ row of W. Geometrically, this means that vector $\vec{z_i}$ is perpendicular to $\vec{z_i}- \vec{p_i}$. Therefore, for every $\vec{p_i}$, $i \in {1,\dots,n_z}$, the corresponding feasible $\vec{z_i}$ trace out a circle with $\frac{w_i}{2} \vec{p_i}$ as the centre. The other linear constraints $P[z] \geq 0$ and $P[z] \geq P[z]$ means that the projection of $\vec{z_i}$ on $\vec{e}$ should be positive and should be larger than the projection of $\vec{p_i}$ on $\vec{e}$.
		\item PSD constraint \\
		As mentioned above, we disregard the PSD constraint for now as we want to analyze it in a worst-case-scenario sense. Added PSD constraint will enforce more dependencies between $x_i$'s and $z_i$'s, and will further decrease relaxation.
	\end{enumerate}{}
	
	Since every $\vec{x_i}$ vector is bounded within a circle, $\vec{p_i}$ will also be bounded within a circle. We could easily give an upper bound on the radius of the circle, namely being $\frac{1}{2}\max \{l_i - u_i\} * \|w_i\|_1$.
	
	We fix $h =  \langle \vec{p_i}, \vec{e} \rangle$ and fix $\theta$, the angle between $\vec{p_i}$ and $\vec{e}$. These two parameters uniquely determine a possible $\vec{p_i}$. Consequently, we want to know $\max (\langle \vec{z_i}, \vec{e}\rangle - \langle \vec{p_i}, \vec{e} \rangle )$, which is the largest possible relaxation for each coordinate $i$ given $h$ and $\theta$.\\
	
	From similar triangles we know that $\max \langle \vec{z_i}, \vec{e}\rangle = \frac{1}{2}h + \frac{h}{2cos(\theta)}$. Therefore for a fixed $h$ and $\theta$ we know 
	\begin{align*}
	\max (\langle \vec{z_i}, \vec{e}\rangle - \langle \vec{p_i}, \vec{e} \rangle ) &= \frac{1}{2}h + \frac{h}{2cos(\theta)} - h \\
	&= \frac{h}{2} \frac{1-cos(\theta)}{cos(\theta)} 
	\end{align*}{}
	
	$h$ is linearly correlated with $\max\{l_i, u_i\}$, therefore by linearly decreasing the limits, i.e. $l' = t *l, u' = t *u, t \in (0,1)$, we get the new $h' = (\alpha t) h$. This term $\alpha$ is the gradient of the linear function $f(l,u) = h$. In this analysis, $\alpha$ usually equals to $\|w_i\|_1$. Thus
	\begin{equation}
	\max_{\text{partitioned}} (\langle \vec{z_i}, \vec{e}\rangle - \langle \vec{p_i}, \vec{e} \rangle ) = \frac{(\alpha t)h}{2} \frac{1-cos(\theta)}{cos(\theta)}
	\end{equation}{}
	
	This equation clearly tells us that relaxation error is linearly correlated with $t$, the factor of limit decrease. Also observe that when $\theta = 0$, there is no relaxation, and as $\theta$ gets larger, the error also grows larger. However, since $h$ and $\theta$ are usually influenced by constraints that we disregard in this analysis, we won't study how partitioning can change the value of $\theta$. Instead, we analyze how linearly decreasing the limits can change the error for all feasible $h$ and $\theta$.
	
	When we have multi-layer connections, we pass the $z$(result of relaxation) of the previous layer to the input $x$ of the next layer. We call $z_p$ the max relaxation with partitioning and $z$ the unpartitioned relaxation, thus $\frac{z_p}{z} = \frac{(\alpha t)h (1+cos(\theta))}{2cos(\theta)} \frac{2cos(\theta)}{h(1+cos(\theta))} = \alpha t$. Therefore, for the next layer, we have a $\alpha t$ decrease in the limits, i.e. $l' = \alpha t l, u' = \alpha t u$. Thus, in the new layer, $h' = (\alpha^2 t)h$. By induction, the final layer has that $h' = (\alpha^{n-1} t)h$, where $L=n$ is the number of layers. However, we recognize here that $\alpha$ is a network parameter, and we can only control $t$.
	
	In conclusion, by controlling $t$, we can achieve linear decrease in relaxation error for all layers. However, depending on the value of $\alpha$, which is controlled by the weight matrix W, we can see different levels of relaxation error decreases in different layers. In particular, if $\alpha < 1$, then the decreasing effect is exponential, exactly what we want. This also tells that the bigger the $h$, therefore the bigger $\|x\|$ is, the better partitioning works.
